Unfolding the Literature: A Review of Robotic Cloth Manipulation

The realm of textiles spans clothing, households, healthcare, sports, and industrial applications. The deformable nature of these objects poses unique challenges that prior work on rigid objects cannot fully address. The increasing interest within the community in textile perception and manipulation has led to new methods that aim to address challenges in modeling, perception, and control, resulting in significant progress. However, this progress is often tailored to one specific textile or a subcategory of these textiles. To understand what restricts these methods and hinders current approaches from generalizing to a broader range of real-world textiles, this review provides an overview of the field, focusing specifically on how and to what extent textile variations are addressed in modeling, perception, benchmarking, and manipulation of textiles. We finally conclude by identifying key open problems and outlining grand challenges that will drive future advancements in the field.

==> bibliography.tex <==
\begin{thebibliography}{00}

\bibitem{Trouve1995a}%1
Trouv\'{e} A. 1995. {\it An approach of pattern recognition through infinite dimensional group action.} Rep. LMENS-95-9, Lab. Math. l'Ecole Norm. Superieure, Paris  

\bibitem{Christensen1996}%2
Christensen G, Miller MI, Rabbit RD. 1995. Deformable templates
using large deformation kinematics. {\it IEEE Trans. Med. Imaging}
5(10):1435--47

\bibitem{Grenander1998}%3
Grenander U, Miller MI. 1998. Computational anatomy: an emerging
discipline. {\it Q. Appl. Math.} 56:617--94

\bibitem{Dupuis1998}%4
Dupuis P, Grenander U, Miller MI. 1998. Variation problems on
flows of diffeomorphisms for image matching. {\it Q. Appl. Math.}
56:587--600

\bibitem{Miller-Younes-2001}%5
Miller MI, Younes L. 2001. Group actions, homeomorphisms, and matching: a general framework. {\it Int. J. Comput. Vis.}
41:61--84

\bibitem{Toga2001}%6
Toga A, Thompson PM. 2001. Maps of the brain. {\it Anat. Rec.}
265:37--53

\bibitem{kapusta2016data}%7
Kapusta A, Yu W,  Bhattacharjee T, Liu C K, Turk G, Kemp C. 2016. {\it  Data-driven haptic perception for robot-assisted dressing.}

\bibitem{chance2017quantitative}
Chance G, Jevtić A, Caleb-Solly P, Dogramadzi S. {\it A quantitative analysis of dressing dynamics for robotic dressing assistance.} Frontiers in Robotics and AI. 2017 May 16;4:13.

\bibitem{sanchez2018robotic}
Sanchez J, Corrales JA, Bouzgarrou BC, Mezouar Y. {\it Robotic manipulation and sensing of deformable objects in domestic and industrial applications: a survey.} The International Journal of Robotics Research. 2018 Jun; 37(7):688-716.

\bibitem{lippi2020latent}
Lippi M, Poklukar P, Welle MC, Varava A, Yin H, Marino A, Kragic D. Latent space roadmap for visual action planning of deformable and rigid object manipulation. In2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS) 2020 Oct 24 (pp. 5619-5626). IEEE.


\bibitem{zhu2021challenges}
Zhu J, Cherubini A, Dune C, Navarro-Alarcon D, Alambeigi F, Berenson D, Ficuciello F, Harada K, Kober J, Li X, Pan J. Challenges and outlook in robotic manipulation of deformable objects. IEEE Robotics \& Automation Magazine. 2022 Feb 25;29(3):67-77. 

\bibitem{huang2023self}
Huang Z, Lin X, Held D. Self-supervised cloth reconstruction via action-conditioned cloth tracking. In2023 IEEE International Conference on Robotics and Automation (ICRA) 2023 May 29 (pp. 7111-7118). IEEE.

\bibitem{matas2018sim}
Matas J, James S, Davison AJ. Sim-to-real reinforcement learning for deformable object manipulation. InConference on Robot Learning 2018 Oct 23 (pp. 734-743). PMLR.

\bibitem{salhotra2022learning}
Salhotra G, Liu IC, Dominguez-Kuhne M, Sukhatme GS. Learning deformable object manipulation from expert demonstrations. IEEE Robotics and Automation Letters. 2022 Jul 1;7(4):8775-82.

\bibitem{ma2022learning}
Ma X, Hsu D, Lee WS. Learning latent graph dynamics for visual manipulation of deformable objects. In2022 International Conference on Robotics and Automation (ICRA) 2022 May 23 (pp. 8266-8273). IEEE.


\bibitem{mo2022foldsformer}
Mo K, Xia C, Wang X, Deng Y, Gao X, Liang B. Foldsformer: Learning sequential multi-step cloth manipulation with space-time attention. IEEE Robotics and Automation Letters. 2022 Dec 15;8(2):760-7.

\bibitem{GRISHANOV201128}
Grishanov S. Structure and properties of textile materials. InHandbook of textile and industrial dyeing 2011 Jan 1 (pp. 28-63). Woodhead Publishing.

\end{thebibliography}


==> sections/08_Conclusions_old.tex <==
\section{DISCUSSION AND FUTURE PERSPECTIVES}
\label{sec:conclusions}

% \TODO{Alberta: Iterate and Shrink}
This section summarizes the main concepts discussed in this review, further identifying open problems and detailing future research directions and grand challenges to foster the development of perception and manipulation skills that generalize to variations of textile properties and manipulation tasks.

\subsection{Synergies}

In previous sections, we examined modeling, perception and manipulation separately. However, there is significant interplay among these domains, impacting generalization and adaptation capabilities. Here, we review some challenges faced by these components individually and how their integration can be beneficial for generalization.

Offloading most computational effort to modeling, such as using analytical models, allows for offline optimization of manipulation trajectories. This reduces the burden on control strategies and perception, as optimal strategies can faithfully execute the task in an open loop~\cite{li2015folding}. While cloth models facilitate transferring to novel tasks~\cite{lin2022learning}, real-world applications require perception techniques to adjust simulator parameters for each real-world object as in Section~\ref{sec::model_real2sim}. This involves estimating object properties from sensors or feedback and replanning to address inaccuracies, making perception crucial for generalization~\cite{longhini2024adafold, longhini2023edonet}.

Model-free learning techniques such as RL and IL shift the computational complexity to manipulation by learning end-to-end from raw data~\cite{hietala2022learning}. While this allows the reduction of the requirements from the perception module, it has to trade sample efficiency and generalizability, which often results in training a single policy for each task, limiting flexibility in varying environments. However, not all the components of a sequential manipulation task need to be learned end-to-end and offloaded to the policy. Sub-tasks within cloth manipulation can be simplified with perception modules. Examples include flattening based on wrinkle~\cite{sun2014heuristic} or grasp point detection~\cite{corona2018active}, and folding plans based on corner alignment, which delegate specific tasks to perception, bypassing the need for extensive learning. 

Conversely, relying solely on perception and heuristic-based approaches hinders generalizability, as it is challenging to design heuristics for all real-world scenarios. Learning policies can address tasks where heuristic-based algorithms fall short. For example, which point to grasp could be addressed by the perception algorithm, how to reach the grasping point can be resolved with a standard planning algorithm, and how to optimize the manipulation once the cloth is grasped can be learned and performed by an end-to-end policy. The underexplored area of switching between learning and heuristic approaches and determining when to use each presents a promising research direction. This is particularly relevant with the advent of foundation models capable of reasoning about semantics and tasks and adapting to rules and human preferences.

\subsection{Open Problems}
% \al{My feeling is that this section is very dense, and it is trying to convey a lot of information. Maybe it is what we want, but if you have a suggestion on how to improve it, let's discuss it.}
To discuss the generalization and adaptation of current methods for cloth manipulation, we provided an overview of fundamental textile properties that contribute to the variations of real-world textiles, highlighting the complexity of understanding their role in manipulation due to the intertwined role of each of them. However, the influence of each textile property in robotic manipulation is still underexplored. Moreover, the extent to which explicit identification of each property is required remains unclear. %For example, while elasticity is a fundamental property for assistive dressing tasks, it plays a marginal role in folding, where stiffness is the pivotal property determining the outcome of the robot's actions. Moreover, explicit identification of mechanical properties may not always be necessary. 
An open avenue for research is identifying a subset of pertinent features for different manipulation task, which can be used to determine the extent to which the textile properties need to be identified. %This understanding can simplify the learning of skills and models. 

Adding to the complexity of identifying and defining the textile properties is the dynamic nature of these properties under varying conditions. Aging of the cloth, as well as wet, dirty, or dry conditions, can alter a textile's behavior, emphasizing the need for continuous sensing and adaptive perception systems in autonomous agents. Moreover, physical attributes like thickness, softness, and durability~\cite{yuan2018active} are typically evaluated alongside semantic descriptors, like smooth, absorbent, hairy, and slippery that humans use to characterize textiles~\cite{chu2013using}. Particularly, with the advances in Large Language Models (LLMs) there is an emerging potential to bridge these descriptive terms with a physical understanding of textile properties~\cite{yu2024octopi}.


One key aspect for manipulating a variety of textiles and addressing the variation of properties is perception.
While interactive perception with different types of sensors and exploratory actions can enhance adaptability and reduce uncertainty in presence of partial observability, it remains underexplored. Multimodal sensing emerges as a pivotal strategy in this context, integrating various sensory inputs like tactile, visual, and auditory data to provide a more holistic understanding of textile properties. 
This approach holds significant potential, as it allows robots to leverage multiple temporal information sources, compensating for the limitations of individual sensors.
% Future advancements in robotic textile manipulation should also focus on exploring interactive perception with different types of sensors and exploratory actions, extending Table~\ref{fig:perception_table}, and integrating multimodal sensory inputs, such as vision and tactile sensing, to enhance adaptability and reduce uncertainty in scenarios where some parts of the cloth are not visible by the camera but reachable to the robot equipped with tactile sensors. This approach is underexplored but holds significant potential, as it allows robots to leverage multiple temporal information sources, compensating for the limitations of individual sensors.





% David: I liked the "A significant observation" :)
A notable finding from our review of manipulation techniques is the limited amount of works demonstrating effective generalization to a wide range of deformable objects, with only a few exploring adaptation techniques.  Most current efforts utilize domain randomization in simulations to enhance sim2real transfer. While promising, these methods often overlook the potential of various domain adaptation techniques that could allow robots to dynamically adjust their manipulation strategies based on real-time environmental feedback and changes in textile properties. %These techniques, such as \al{some citations here}, hold the potential to enable robots to adapt their manipulation strategies in real-time to cope with unexpected changes in the textile properties or environment. 
%Adaptation enables models to adjust dynamically based on feedback from the environment.
Similarly, the use of state-of-the-art models such as diffusion models, in combination with imitation learning techniques, has predominantly focused on rigid objects due to the complexity of state estimation and high-dimensional state spaces of textiles. This leaves open questions about their applicability to deformable objects and the challenges of deploying these methods without assuming rigidity. 

%Developing universal models or policies that can handle multiple textile manipulation tasks, rather than task-specific models, remains relatively unexplored. The introduction of LLMs also presents an opportunity to simplify task specification and the planning of sequential tasks of textiles, as well as merging physical textile attributes with human-interpretable semantic descriptors.

Building on the necessity for improved generalization in manipulation techniques, benchmarking, standardization and datasets emerge as essential yet challenging areas. The diversity of robotic embodiments, sensor configurations, and test sets, complicates the comprehensive comparison of approaches and algorithms. Specifically, the development of universally applicable testing datasets is hindered by issues like stock availability and the difficulties associated with measuring properties accurately. Although there has been some progress towards creating standardized test sets and benchmarks, these continue to be significant open problems within the field. Additionally, a major challenges in dataset availability and scalability  is accurately labeling the deformable object dataset, which limits their widespread distribution and application.

\subsection{Grand Challenges}
To push the boundaries of robotic manipulation of textiles, we identify the following critical challenges that the research community should address:

% \begin{itemize}
% Perception of new textiles: Develop methods to accurately estimate key properties of new textiles. This requires not only understanding the properties of interest but also employing combinations of sensing and exploratory procedures designed to identify these properties effectively.

\textbf{Perception of properties of novel objects:} Develop advanced methods for accurately estimating key physical and semantic properties of new textiles. This challenge requires integrating sophisticated sensing technologies and exploratory procedures to identify these properties effectively. Achieving this would enhance robotic manipulation, enabling robots to adaptively handle a diverse range of textiles.

% \item Multi-modal, Multi-task, Multi-embodiment Generalist Agent: Create an agent capable of addressing multiple tasks in unknown environments, particularly those involving the manipulation of deformable objects and performing assistive tasks with humans in the loop. Challenges include learning to autonomously adapt to complex situations and acquiring skills from minimal human demonstrations.

\textbf{Multi-modal, Multi-task, Multi-embodiment Generalist Agent: } Develop an agent capable of addressing multiple tasks in unknown environments, especially those involving the manipulation of deformable objects and assistive tasks with humans in the loop. This requires the agent to autonomously adapt to complex situations and acquire skills from minimal human demonstrations, leveraging multi-modal sensory inputs and versatile embodiment strategies. Achieving this would significantly advance robotic flexibility and effectiveness in diverse real-world applications.

% \item Datasets and Benchmarking: Address the difficulties in creating comprehensive datasets due to the high-dimensional state space and degrees of freedom. A well-annotated dataset encompassing the 2D state across various dynamic interactions and labeled with relevant features and properties would greatly benefit the community. Additionally, designing experimental benchmarking procedures for textile objects that can be standardized across institutions, considering stock availability and object variations, is crucial for progress.
% \end{itemize}

\textbf{Datasets and Benchmarking:} Address the challenges in creating comprehensive datasets for high-dimensional state spaces and degrees of freedom in robotic manipulation. Develop a well-annotated dataset that captures 2D or 3D states across diverse, dynamic interactions labeled with relevant features and properties. Additionally, design standardized experimental benchmarking procedures for textile objects, considering stock availability and object variations, to facilitate consistent progress across research institutions. Achieving this will significantly enhance the community's ability to develop and compare advanced robotic systems.



% Grand challenges to discuss
% \begin{itemize}
%     \item Characterization and Perception of Textile Properties: there are different levels of abstractions of properties that we do not consider but that are relevant in real-world applications. Their relevance and how they are perceived contain a lot of potential future directions to explore.
%     \item Manipulation techniques: there is a lot for rigid in terms of diffusion as well as adaptation techniques, but not for deformable. \al{What about modeling? Analytical models will never be good, but we could explore better ways to exploit them as priors, and this direction has definitely gained some interest recently, also thanks to differentiable simulators.}
%     \item Variations of tasks: some tasks are not addressed.
%     \item Benchmarking, standardization.
% \end{itemize}







